SCAR: Strong Consistency using Asynchronous Replication with Minimal Coordination

Data replication is crucial in modern distributed systems as a means to provide high availability. Many techniques have been proposed to utilize replicas to improve a system's performance, often requiring expensive coordination or sacrificing consistency. In this paper, we present SCAR, a new distributed and replicated in-memory database that allows serializable transactions to read from backup replicas with minimal coordination. SCAR works by assigning logical timestamps to database records so that a transaction can safely read from a backup replica without coordinating with the primary replica, because the records cannot be changed up to a certain logical time. In addition, we propose two optimization techniques, timestamp synchronization and parallel locking and validation, to further reduce coordination. We show that SCAR outperforms systems with conventional concurrency control algorithms and replication strategies by up to a factor of 2 on three popular benchmarks. We also demonstrate that SCAR achieves higher throughput by running under reduced isolation levels and detects concurrency anomalies in real time.

==> replication.tex <==
%!TEX root = main.tex

